Estimating WebRTC Video QoE Metrics Without Using Application Headers

The increased use of video conferencing applications (VCAs) has made it critical to understand and support end-user quality of experience (QoE) by all stakeholders in the VCA ecosystem, especially network operators, who typically do not have direct access to client software. Existing VCA QoE estimation methods use passive measurements of application-level Real-time Transport Protocol (RTP) headers. However, a network operator does not always have access to RTP headers in all cases, particularly when VCAs use custom RTP protocols (e.g., Zoom) or due to system constraints (e.g., legacy measurement systems). Given this challenge, this paper considers the use of more standard features in the network traffic, namely, IP and UDP headers, to provide per-second estimates of key VCA QoE metrics such as frames rate and video resolution. We develop a method that uses machine learning with a combination of flow statistics (e.g., throughput) and features derived based on the mechanisms used by the VCAs to fragment video frames into packets. We evaluate our method for three prevalent VCAs running over WebRTC: Google Meet, Microsoft Teams, and Cisco Webex. Our evaluation consists of 54,696 seconds of VCA data collected from both (1), controlled in-lab network conditions, and (2) real-world networks from 15 households. We show that the ML-based approach yields similar accuracy compared to the RTP-based methods, despite using only IP/UDP data. For instance, we can estimate FPS within 2 FPS for up to 83.05% of one-second intervals in the real-world data, which is only 1.76% lower than using the application-level RTP headers.

==> sections/ethics.tex <==
\section{Ethics}
The household network traces used in this paper are collected after
obtaining approvals from our Institutional Review Board (IRB).
We prioritize the protection of user privacy and take extensive measures
to ensure it. \textcolor{blue}{The Raspberry Pi devices used for this study were connected to the home router in a wired manner. All VCA calls were conducted between the Raspberry Pi and a cloud-based server. Therefore, all our network traces contain information relevant to the end-to-end path between the Raspberry Pi and the VCA SFU}. Furthermore, we remove any personally identifiable information, such as physical address and demographics,
before analyzing the data. The remaining datasets used
in this paper are collected within controlled lab setting and do not pose any privacy-related issues.
